Capturing Homomorphism-Closed Decidable Queries with Existential Rules

Existential rules are a very popular ontology-mediated query language for which the chase represents a generic computational approach for query answering. It is straightforward that existential rule queries exhibiting chase termination are decidable and can only recognize properties that are preserved under homomorphisms. In this paper, we show the converse: every decidable query that is closed under homomorphism can be expressed by an existential rule set for which the standard chase universally terminates. Membership in this fragment is not decidable, but we show via a diagonalisation argument that this is unavoidable.

==> 1-introduction.tex <==
%\section{Introduction}
%\label{section:introduction}

\smallskip
The main goal of this paper is to show the following:

\begin{theorem}
Consider a Boolean query \Query that is decidable and homomorphism-closed.
Then, there is \cbadded{an existential} rule set \RuleSet that expresses \Query and is chase-terminating.
\end{theorem}

The above result follows from Lemmas~\ref{lemma:expressivity}, \ref{lemma:same-expressivity}, \ref{lemma:chase-termination}, and \ref{lemma:michaels-lemma}.
We obtain the following corollary.

\begin{corollary}
\cbadded{When used as an ontology language, no decidable FOL fragment is more expressive than chase-terminating existential rules.}
%Add a result stating that the chase-terminating fragment is the most expressive FOL with respect to our notion of expressivity.
\end{corollary}

%\sru{As discussed before, this is a highly misleading statement, since it uses a very non-standard notion of FOL-expressivity. I would therefore advocate to remove it, as it will most certainly get us into serious trouble upon reviewing, even if we introduce ``our'' idea of FOL-expressibility.}


Remarks to be added:
\begin{itemize}
%\item Note that we cannot express queries that are undecidable or not homomorphism-closed in First-order logic.
\item Discuss results on the limits of the expressivity of detectable and semi-detectable languages.
\end{itemize}




==> back-propagation.tex <==
\section{Back Propagation}
Assumptions:
\begin{itemize}
 \item $\varphi_i(w,w',\mathbf{t})$ is a conjunctive query with free variables $w,w'$ and $\mathbf{t}$, such that the only variables that may appear in an affected position in $\varphi_i$ are $w$ and $w'$;
 \item $p_{g_i}$ is a fresh predicate for any $i$.
\end{itemize}



\begin{definition}[Conditional Successors]
Let $\{\varphi_1,\ldots,\varphi_n\}$ be a set of conditional queries. A set of conditional successors for an element $w$ is a set $\{w_1,\ldots,w_n\}$ for which there exists $\mathbf{t}$ such that for all $i$, $I \models \varphi_i(w,w_i,\mathbf{t})$.
\end{definition}

\begin{definition}
 An individual is validated if it belongs to the smallest set of elements that contains all the elements such that $p_g(w) \in I$, and that contains any $w$ that has a set of conditional successors that are all validated.
  \end{definition}

\begin{definition}
 A set of rules $\Sigma_{\mathsf{bp}}$ is a back propagation implementation if for any admissible instance, it holds that 
 $\{w \mid I,\Sigma_{\mathsf{bp}} \models p_g(w)\}$ is the set of validated individuals. 
\end{definition}


Abstract Implementation:

\begin{itemize}
 \item $\varphi_i(w,w',\mathbf{t}) \wedge p_g(w') \rightarrow p_{g_i}(w,\mathbf{t})$
 \item $\bigwedge_i p_{g_i}(w,\mathbf{t}) \rightarrow p_g(w)$
\end{itemize}


We will use two sets of conditional queries:
\begin{itemize}
 \item $\{\varphi_{<}(w,w',x,y),\varphi_{>}(w,w',x,y),\varphi_{=}(w,w',x,y)\}$
 \item $\{\varphi_{p}(w,w',\mathbf{t}),\varphi_{\bar{p}}(w,w',\mathbf{t}\}$
\end{itemize}






\section{Another Try at Formalizing the Treeish Part}

Let $D$ be a database, $\Sigma$ be a ruleset, $\mathcal{I}$ be a model of $D$ and $\Sigma$.

We define:
\begin{itemize}
 \item $\mathsf{order}(a) = \{ x \leq y \mid (a,x,y) \in \leq^\mathcal{I}\} \cup \{ x = y \mid (a,x,y) \in =^\mathcal{I}\}$
 \item $\mathsf{world}(a) = \{p(t) \mid (a,t) \in p^\mathcal{I}\}$.
\end{itemize}


\paragraph{Database Completion}
$\Sigma_{dbc}$ is a database completion implementation for a set of predicates $\mathcal{P} \dot\cup \{\leq,=\}$ if
\begin{itemize}
 \item for any model $\mathcal{I}$ of $D,\Sigma_{dbc}$ (and $\Sigma$ on ??) such that $D$ is on $\mathcal{P}$, there exists a $a \in dom(\mathcal{I})$ s.t. $a \in \mathsf{World}^\mathcal{I}$ and $D \subseteq \mathsf{world}(a)$;
 \item for any model $\mathcal{I}$ of $D,\Sigma_{dbc}$ (and $\Sigma$ on ??) such that $D$ is on $\mathcal{P}$, for any $a \in \mathsf{World}^\mathcal{I}$, for any $p \in \mathcal{P}\dot\cup\{\leq,=\} \cup \bar{\mathcal{P}}$, for any tuple of correct arity $t$,  there exists $a'$ such that $(a,a',t)\in \mathsf{child}_p^\mathcal{I}$ and $a' \in \mathsf{World}^\mathcal{I}$
 \item for any model of $D,\Sigma,\Sigma_{dbc}$ (and $\Sigma$ on ??) such that $D$ is on $\mathcal{P}$, if $(a,a',t) \in \mathsf{child}_p^\mathcal{I}$, then $\mathsf{world}(a)\cup p(t) \subseteq \mathsf{world}(a')$
 \item there exists a model $\mathcal{I}$ of $D, \Sigma, \Sigma_{dbc}$ in which:
 \begin{itemize}
 \item for all $a,a',t \in Dom(\mathcal{I})$, $(a,a',t) \in \mathsf{child}_p^\mathcal{I}$ implies that $\mathsf{world}(a)\cup p(t) = \mathsf{world}(a')$
 \item there exists $a$ such that $\mathsf{world}(a) = D$
 \end{itemize}
\end{itemize}

\paragraph{Cycle Check}
$\Sigma_{cc}$ is a cycle check implementation if for any instance $D$ on $\mathcal{P} \dot\cup\{\leq,=\}$, $D, \Sigma_{cc} \models \mathsf{goal}$ if and only if there is a cycle in the order described by $\leq$ and $=$.

\paragraph{Consistency Check}
$\Sigma_{cons}$ is a consistency check implementation if for any instance $D$ on $\mathcal{P} \dot\cup \bar{\mathcal{P}}$, $D,\Sigma_{cons} \models \mathsf{goal}$ if and only if there exists $t$ and $p$ such that $p(t) \in D$ and $\bar{p}(t) \in D$.

\paragraph{Contextualisation}
Contextualisation is a transformation of a rule set which adds to every predicate a first position, which is filled in every rule by the same fresh variable $w$. Contextualisation of cycle check and consistency check should provide us with what we want.

\paragraph{Back Propagation}
$\Sigma_{bp}$ is a back propagation implementation for $p$ if for any instance $D$, for any ruleset $\Sigma$ (whose output predicate include a unary $\mathsf{goal_t}$ and a unary $\mathsf{goal_c}$) the following holds:

\begin{itemize}
 \item if $\mathcal{I}$ is a model of $D,\Sigma, \Sigma_{bp}$, then for any $a$, if there exists $a'$ and $a''$ such that $(a,a',t) \in \mathsf{child}_p^\mathcal{I}$, $(a,a'',t) \in \mathsf{child}_{\bar{p}}^\mathcal{I}$, $a' \in \mathsf{goal}^\mathcal{I}$ and $a'' \in \mathsf{goal}^\mathcal{I}$, then $a \in \mathsf{goal}^\mathcal{I}$
 \item if $\mathcal{I}$ is a model of $D,\Sigma, \Sigma_{bp}$, if $a \in \mathsf{goal_t}^\mathcal{I}$ or $a \in \mathsf{goal_c}^\mathcal{I}$, then $a \in \mathsf{goal}^\mathcal{I}$;
 \item there exists a model $\mathcal{I}$ in which $a \in \mathsf{goal}^\mathcal{I}$ iff at least one of the following holds: 
 \begin{itemize}
 \item $a \in \mathsf{goal_t}^\mathcal{I}$, 
 \item $a \in \mathsf{goal_c}^\mathcal{I}$,
 \item there exists $a',a''$ such that $(a,a',t) \in \mathsf{child}_p^\mathcal{I}$, $(a,a'',t) \in \mathsf{child}_{\bar{p}}^\mathcal{I}$, $a' \in \mathsf{goal}^\mathcal{I}$ and $a'' \in \mathsf{goal}^\mathcal{I}$.
\end{itemize}
\end{itemize}

\begin{center}
\begin{figure}
\begin{tikzpicture}%[every node/.append style={sloped, scale=.8}]

\node at (0,0) (completion) {$\Sigma_{dbc}$};
\node at (-4,-2) (consistency) {$\Sigma_{cc},\Sigma_{cons}$};
\node at (-2,-3) (brake) {$\Sigma_{eb}$};
\node at (0,-4) (serial) {$\Sigma_{serial}$};
\node at (0,-6) (simul) {$\Sigma_{simul}$};
\node at (0,-8) (propagation) {$\Sigma_{bp}$};

\draw (completion) edge[->] node[left] {$\{p,\bar{p},=,\leq\}$} (consistency);
\draw (completion) edge[->] node[left] {$\{p,\bar{p},=,\leq\}$} (serial);
\draw (completion) edge[->,bend left] node[right] {$\mathsf{child_p}$} (propagation);
\draw (consistency) edge[->] node[left] {$\mathsf{goal_c}$} (propagation);
\draw (consistency) edge[->] node[right] {$\mathsf{goal_c}$} (brake);
\draw (brake) edge[->] (serial);
\draw (brake) edge[<->] (simul);
\draw (serial) edge[->] (simul);
\draw (simul) edge[->] node[left] {$\mathsf{goal_t}$} (propagation);


\end{tikzpicture}
\caption{Map of interfaces and of their communication means}
\end{figure}
\end{center}

\begin{center}
\begin{figure}
\begin{tikzpicture}%[every node/.append style={sloped, scale=.8}]

\node at (0,0) (completion) {$\Sigma_{dbc}$};
\node at (-4,-3) [draw,thick,minimum width = 2cm, minimum height=1cm] (consistency) {$\Sigma_{cc},\Sigma_{cons}$};
\node at (-5.5,-3) (brake) {$f_c$};
\node at (-1,-4) (serial) {$\Sigma_{serial}$};
\node at (-1,-6) (simul) {$\Sigma_{simul}$};
\node at (0,-8) (propagation) {$\Sigma_{bp}$};

\node (rect) at (-1,-5) [draw,thick,minimum width=2cm,minimum height=3cm] {};
\node (fonction) at (0.5,-5) {$f_b\circ f_c$};

\draw (completion) edge[->] node[left] {$\{p,\bar{p},=,\leq\}$} (consistency);
\draw (completion) edge[->] node[left] {$\{p,\bar{p},=,\leq\}$} (rect);
\draw (completion) edge[->,bend left] node[right] {$\mathsf{child_p}$} (propagation);
\draw (consistency) edge[->, bend right] node[left] {$\mathsf{goal_c}$} (propagation);
\draw (consistency) edge[->] node[above] {$\mathsf{goal_c}$} (rect);
%\draw (brake) edge[->] (serial);
%\draw (brake) edge[<->] (simul);
\draw (serial) edge[->] (simul);
\draw (rect) edge[->] node[left] {$\mathsf{goal_t}$} (propagation);


\end{tikzpicture}
\caption{Another map, with contextualisation and emergency brake as functions.}
\end{figure}
\end{center}



==> emergency-brake.tex <==
\newcommand{\defeq}{:=}

\section{Emergency Brake}

\begin{definition}
For a rule set $\Sigma$, let
$\mathsf{edb}(\Sigma)$ be the set of all predicate symbols in $\Sigma$ that
do not occur in the head of a rule, and let $\mathsf{idb}(\Sigma)$ be the
set of all predicate symbols in $\Sigma$ that occur in some rule head.
Moreover, let $\mathsf{pred}(\Sigma)\defeq\mathsf{edb}(\Sigma)\cup\mathsf{idb}(\Sigma)$.
We also use $\mathsf{pred}$ on databases and queries.

A database $D$ is a \emph{database for $\Sigma$} if $\mathsf{pred}(D)\subseteq\mathsf{edb}(\Sigma)$.
A query $q$ is a \emph{query for $\Sigma$} if $\mathsf{pred}(q)\subseteq\mathsf{pred}(\Sigma)$.

A rule set $\Pi$ is \emph{unaffected by} $\Sigma$ if 
$\mathsf{pred}(\Pi)\cap\mathsf{pred}(\Sigma)\subseteq\mathsf{edb}(\Sigma)\}$
% 
% We write $\Sigma[\mathbb{I},\mathbb{O}]$ to denote a set of rules $\Sigma$
% together with two finite, disjoint sets of \emph{input predicates} $\mathbb{I}$ and
% \emph{output predicates} $\mathbb{O}$, where we require that predicates of $\mathbb{I}$ do
% not occur in rule heads of $\Sigma$.
% $\Sigma$ may contain further \emph{auxiliary predicates} that
% do not occur in $\mathbb{I}\cup\mathbb{O}$.
% 
% Given rule sets $\Sigma[\mathbb{I},\mathbb{O}]$ and $\Sigma'[\mathbb{I}',\mathbb{O}']$,
% $\Sigma\uplus\Sigma'$ is the 
\end{definition}

\begin{definition}
Consider a rule set $\Sigma$ and a nullary predicate $\mathsf{halt}\notin\mathsf{pred}(\Sigma)$.
We introduce auxiliary predicates that are not in $\mathsf{pred}(\Sigma)$:
(i) unary predicates $\mathsf{eb}$ and $\mathsf{r}$, 
(ii) for all $p\in\mathsf{idb}(\Sigma)$, a predicate $\hat{p}$ of the same arity, and
(iii) for all rules $\rho\in\Sigma$, a predicate $b_\rho$ with arity the size of the frontier of $\rho$.
Now the set $\mathsf{brake}(\Sigma,\mathsf{halt})$ consists of the following rules:
\begin{itemize}
\item The rules
\begin{align}
 &\to\exists v.\mathsf{eb}(v)\wedge \Omega^v_\Sigma\\
 \mathsf{halt}\wedge\mathsf{eb}(v)  &\to \mathsf{r}(x)
\end{align}
where $\Omega^v_\Sigma$ is the conjunction of all atoms of the form $\hat{p}(v,v,\ldots,v)$ for predicates $p\in\mathsf{idb}(\Sigma)$.
\item For every $p\in\mathsf{idb}(\Sigma)$, a rule
\begin{align}
\hat{p}(\vec{x})\wedge \bigwedge_{x\in\vec{x}} \mathsf{r}(x) & \to p(\vec{x}).
\end{align}
\item For every rule $\rho: \varphi[\vec{x},\vec{y}]\to\exists\vec{z}.\psi[\vec{x},\vec{z}]$, two rules
\begin{align}
\varphi[\vec{x},\vec{y}]\wedge\mathsf{eb}(v) &\to b_\rho(\vec{x})\wedge\hat{\psi}[\vec{x},\vec{z}/v]\wedge \bigwedge_{x\in\vec{x}} \mathsf{r}(x) \\
b_\rho(\vec{x}) & \to \exists\vec{z}.\hat{\psi}[\vec{x},\vec{z}]\wedge\bigwedge_{z\in\vec{z}} \mathsf{r}(z)
% \psi\wedge\mathsf{eb}(v)\to\exists\vec{z}.\phi\wedge \nu_{\vec{z}}\wedge\phi_v 
\end{align}
where $\hat{\psi}$ is $\psi$ with all predicates $p$ replaced by $\hat{p}$,
and $\hat{\psi}[\vec{x},\vec{z}/v]$ is obtained by replacing each $z\in\vec{z}$ with $v$.
% 
% where $v\notin\vec{x}\cup\vec{z}$,
% $\nu_{\vec{z}}=\bigwedge_{z\in\vec{z}}\mathsf{r}(z)$, and
% $\phi_v= \bigwedge_{\alpha\in\phi} \alpha[\vec{z}/v]$ is the conjunction of atoms in $\phi$ with all variables of $\vec{z}$ replaced by $v$
% (atoms $\alpha$ without variables from $\vec{z}$ are as in $\phi$ and can be omitted).
%
\end{itemize}
\end{definition}

% \begin{definition}
% A rule set $\Pi$ is \emph{compatible} with $\mathsf{brake}(\Sigma,\mathsf{halt})$
% if $\mathsf{pred}(\Pi)\cap\mathsf{pred}(\Sigma)\subseteq\mathsf{edb}(\Sigma)\cup\{\mathsf{halt}\}$.
% \end{definition}

\begin{proposition}
The rule set $\mathsf{brake}(\Sigma,\mathsf{halt})$ is of polynomial size with respect
to $\Sigma$, and we have
$\mathsf{edb}(\mathsf{brake}(\Sigma,\mathsf{halt})) = \mathsf{edb}(\Sigma)\cup\{\mathsf{halt}\}$ and
$\mathsf{idb}(\mathsf{brake}(\Sigma,\mathsf{halt})) = \mathsf{idb}(\Sigma)\cup\{\mathsf{r},\mathsf{eb}\}\cup\{\hat{p}\mid p\in\mathsf{idb}(\Sigma)\}$.
\end{proposition}

\begin{proposition}
Consider a rule set $\Sigma$ and a predicate $\mathsf{halt}\notin\mathsf{pred}(\Sigma)$.
For every rule set $\Pi$ unaffected by $\mathsf{brake}(\Sigma,\mathsf{halt})$,
and every database $D$ and BCQ $q$ for $\Sigma\cup\Pi$, we have that:
\begin{itemize}
\item if $\Sigma,\Pi,D\models q$ then $\mathsf{brake}(\Sigma,\mathsf{halt}),\Pi,D\models q$,
\item if $\mathsf{brake}(\Sigma,\mathsf{halt}),\Pi,D\models q$ then $\Sigma,\Pi,D\models q\vee \mathsf{halt}$,
\item if the standard chase universally terminates over $\Sigma\cup\Pi\cup D$ then it universally terminates over $\mathsf{brake}(\Sigma,\mathsf{halt})\cup\Pi\cup D$,
\item if the standard chase universally terminates over $\Pi\cup D$ and $\Sigma,\Pi,D\models \mathsf{halt}$ then the standard chase universally terminates over $\mathsf{brake}(\Sigma,\mathsf{halt})\cup\Pi\cup D$.
\end{itemize}
\end{proposition}

